Atomistic-Level Analysis of Nanoindentation-Induced Plasticity in Arc--Melted NiFeCrCo Alloys: The role of stacking faults

Concentrated solid solution alloys (CSAs) have attracted attention for their promising properties; however, current manufacturing methods face challenges in complexity, high costs, and limited scalability, raising concerns about industrial viability. The prevalent technique, arc melting, yields high-purity samples with complex shapes. In this study, we explore nanoindentation tests at room temperature where arc-melted samples exhibit larger grain sizes, diminishing the effects of grain boundaries on the results. Motivated by these findings, our investigation focuses on the atomistic-level exploration of plasticity mechanisms, specifically dislocation nucleation and propagation during nanoindentation tests. The intricate chemistry of NiFeCrCo CSA influences pile-ups and slip traces, aiming to elucidate plastic deformation by considering both pristine and pre-existing stacking fault tetrahedra. Our analysis scrutinizes dynamic deformation processes, defect nucleation, and evolution, complemented by stress-strain and dislocation densities-strain curves illustrating the hardening mechanism of defective materials. Additionally, we examine surface morphology and plastic deformation through atomic shear strain and displacement mappings. This integrated approach provides insights into the complex interplay between material structure and mechanical behavior, paving the way for an enhanced understanding and potential advancements in CSA applications.

==> sections/dislocations.tex <==
\subsection{Dislocation nucleation}
\label{subsec:disloc}



In general, dislocation glide occurs in the closest--packed $\langle 
111 \rangle$ directions for BCC metals with Burgers vector 
$b = 1/2 \langle111\rangle$, and slip planes belong to the \{110\}, \{112\}.
To analyze the atomic structure during nanoindentation test 
which provides information about the mechanisms of dislocation 
nucleation and evolution \cite{DeBacker2017}, we use OVITO \cite{ovito} 
with the DXA package \cite{Stukowski_2012} to identify  dislocations 
into several dislocation types according to their Burgers vectors as: 
$1/2 \langle 111 \rangle$, $\langle 100 \rangle$, and 
$\langle 110 \rangle$ dislocation types with their corresponding
dislocation density, $\rho$, defined as
\begin{equation}
    \rho = \frac{l_{klm}}{V_D},
\end{equation}
where $l_{klm}$ is the dislocation length of each type,
by using a hemispherical radius of the plastic zone of 
$r_{\rm pz} = a_{\rm pz}\left[r^2 -(r-h)^2 \right]^{1/2}$ with 
$a_{\rm pz} = 1.9$ and the total volume equals to the hemispherical 
volume excluding the volume displaced by the indenter tip as 
$V_D = \left(2\pi r_{\rm pz}^3/3 \right) -
\left(\pi h^2 (r-h)/3\right) $, with $r$ as the indenter radius 
and $h$ the indentation depth. 
Excluding pile up or sink in effects in this model \cite{BEGAU2012711}.



\begin{figure*}[!t]
   \centering
  % \includegraphics[width=0.40\textwidth]{Figures/dislocationNucleation.png}
  \includegraphics[width=0.9\textwidth]{Figures/Fig6.png}
   \caption{(Color on-line). Visualization of the dislocation 
   nucleation and evolution at depth $z=0.9a$. 
   }
   \label{fig:visdislInit}
\end{figure*}


\begin{figure*}[!t]
   \centering
  % \includegraphics[width=0.40\textwidth]{Figures/dislocationNucleation.png}
  \includegraphics[width=0.9\textwidth]{Figures/Fig7.png}
   \caption{(Color on-line). Visualization of the dislocation 
   nucleation and evolution at at depth $z=1.22a$, using all approaches. 
   Shear dislocation loops are 
   nucleated at the maximum indentation depth in the case of all potentials.}
   \label{fig:visdisl}
\end{figure*}



%by using the Dislocation Extraction Analysis (DXA) tool 
%\cite{ovito,Stukowski_2012}. 
Fig. \ref{fig:DislocationDensity} shows dislocation densities as 
a function of normalized indentation depth for 300 and 77 K of 
(001) W samples.
Oscillations are observed in the loading process
for the densities of both $\langle 111 \rangle$ and total dislocations at both 
temperatures, with minima occurring at 0.9 and 1.1 z/$a$ points, 
where prismatic loops were observed to nucleate. 
It is worth noting that the different potentials we used yielded 
different results for the nucleation and evolution of dislocation junctions 
at the $\langle 100 \rangle$ plane, where a good representation of 
dislocation glide is important. This mechanisms is poorly represented by 
the EAM and EAM/ZBL methods.
We also observed that the formation of this type of defect is common 
under the indenter tip, where the interaction or dissociation of 
$1/2 \langle 111 \rangle$ dislocations can lead to the nucleation 
of dislocation junctions as: $1/2 \langle 111 \rangle$ + 
$1/2 \langle \bar{1} \bar{1}1 \rangle$ = $\langle 001 \rangle$, and
other symmetrically geometrical combinations. 
We observed temperature effects at the point where dislocations begin
to nucleate, this difference is likely due to the increased 
thermal motion of the atoms in the top layer at the higher temperature, 
which affects the dislocations mechanisms to nucleate and propagate 
through the material. 
In the SM, we report results for the (011) and (111) W matrices 
with results than those for (001) W.
%The tabGAP approach seems to model this mechanism properly. 
%due to its parametrization to DFT results.

We visualize the dislocation network nucleated at a depth of z=0.9$a$ in Fig \ref{fig:visdislInit} where initial half loops noted
and z=1.22$a$ in Fig \ref{fig:visdisl} where prismatic loops evolve 
through the sample, at 77 and 300 K sample temperature. 
For BCC materials with a (001) orientation, it is well known that the 
nucleation of prismatic loops is initiated by the formation of shear loops
after the yield point \cite{REMINGTON2014378,JavVarilla}, which then propagate 
along the expected $\langle 111 \rangle$ slip directions.
This mechanism was observed in our MD simulations using MEAM, ABOP, 
and particularly tabGAP (Fig. \ref{fig:visdislInit} c-d). 
Temperature effects on this mechanism are associated with the faster 
propagation of shear loops at lower temperatures, 
this is due to the more stable lattice positions of the W atoms 
during the loading process, which leads to the more efficient nucleation
of prismatic loops (See Fig. \ref{fig:visdisl} c-d). 
As the indenter tip goes deeper into the sample, the shear loops expand 
through the advancement of edge dislocations, while the screw dislocations 
can undergo limited cross-slip, as seen in the simulations using MEAM, 
ABOP, and tabGAP. 
This cross-slip of the screw dislocations eventually leads to a pinch--off 
action, resulting in the formation of prismatic loops. 
It is worth noting that the edge dislocations cannot undergo 
cross--slip.
As plastic deformation proceeds during the loading process, the formed 
prismatic loop advances and the process of shear loop formation and cross--slip 
repeats itself underneath the indenter tip. 
We noticed that among the different potentials we used, tabGAP simulations
provided the most accurate modeling of this mechanism, 
showing good qualitative agreement with the results that are expected 
to be observed in experiments \cite{BEAKE201863,1998562}.

\begin{table}[b!]
    \centering
    \caption{Average number of dislocation loops nucleated at the 
    maximum indentation depth for W by different potentials. 
    Results for temperatures of 300 K and 77 K. }
    %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{crrrrrr}
    \hline
            &   \multicolumn{2}{c}{(001)} & \multicolumn{2}{c}{(011)} & 
            \multicolumn{2}{c}{(111)} \\
    Potentials & 300K & 77K & 300K & 77K &  300K & 77K \\
    \hline
     EAM    &   1   & 2 & 3 & 4 & 1 & 2 \\
    EAM/ZBL &   -  & -  & 2 & 3 & 1 & 2 \\
    MEAM     & 3   & 4  & 6  &  9 & 4 & 5  \\
    ABOP    &  4 & 6 & 5 & 6 & 6 & 7 \\
    tabGAP   & 4 & 6 & 5 & 7 & 6 & 8 \\
    \hline
    \end{tabular}
    %}
    \label{tab:loops}
\end{table}



%The [011] crystal orientation, at a depth of $0.5$ nm, 
%a half loop is nucleated by all the potentials
%with a burger vector $1/2 \langle 111 \rangle$ where EAM 
%potentials mainly nucleate a $\langle 100 \rangle$ junction. 
%In addition, for the [111] orientation, 
It is well known that dislocation glide in BCC metals is 
mainly governed by the Peierls barrier, which measures the 
stress that needs to be applied in order to move a dislocation
core to the next atomic valley in the glide plane. 
Moreover, the Peierls barrier is smaller for edge dislocations
than for screw dislocations, where the BCC metal plasticity
is dominated by the sluggish glide of screw dislocation segments,
as shown by our MD simulations \cite{PhysRevMaterials.4.023601,PhysRevMaterials.2.073608}.
Thus, the ‘lasso‘ mechanism is observed by all methods for (111) W, 
suggesting that the main dislocation nucleation
mechanism remains analogous to other BCC metals \cite{JavVarilla,DOMINGUEZGUTIERREZ2021141912} with a difference 
on the number loops nucleated by each approach. 
In Tab. \ref{tab:loops} we present the number 
of prismatic loops nucleated at the maximum indentation depth, 
quantified for all the potentials we tested at different temperatures. 
We noticed that ABOP and tabGAP are capable to model the nucleation 
of dislocation loops on the expected $\langle 111 \rangle$ and 
$\langle 112 \rangle$ slip directions.
The visualization of the dislocation dynamics during the nanoindentation 
test for both the (011) and (111) orientations can be found in 
the supplementary material \cite{SM}.

==> sections/slipTrace.tex <==
\subsection{Nanoindentation–induced plastic patterning }
\label{sec:results_dis}





The formation of slip traces at the surface is an important aspect
of the crystal plasticity process that occurs during a nanoindentation
test, as these traces provide evidence of the underlying dislocation
glide processes occurring in the subsurface.
As shown in Fig. \ref{fig:pattern300}, the four
$\langle 111 \rangle$ slip directions that occur at 300 K 
temperature lead to the formation of surface pile--ups 
with four--fold symmetry. 
This figure provide a visualization of this process at 
the maximum indentation depth by using different approaches. 
The figure includes a color palette that indicates the magnitude
of the displacement, revealing that the pile-ups form around the 
indenter mark in the shape of a four-folded rosette due to the (001) 
orientation of the W matrix, as expected for BCC metals on a (001) 
orientation. This has been reported experimentally for tungsten by
Argus images reported by H. Yu et al. \cite{YU2020135}, where 
the surface morphology shows four--fold slip traces on the 
$(1\bar{1}0)$ and (110) planes. 
Moreover, Large-scale MD simulations 
for $\alpha$-Fe \cite{VARILLAS2017431} have also demonstrated similar 
pile-ups resulting from the slip directions.

\begin{figure}[!t]
   \centering
  % \includegraphics[width=0.40\textwidth]{Figures/dislocationNucleation.png}
  \includegraphics[width=0.48\textwidth,height=0.48\textwidth]{Figures/Fig8.png}
   \caption{(Color on-line). Visualization of the formation of pile-ups 
   and slip traces for the indented [001] W sample at the maximum depth (3nm). 
   The surface morphology for ABOP and tabGAP show four--fold slip 
   traces on the $(1\bar{1}0)$ and (110) planes in 
   good agreement with experimental findings \cite{YU2020135}. 
      }
   \label{fig:pattern300}
\end{figure}
 
In Fig. \ref{fig:pattern77}, we present the results
of von Mises strain atomic mapping at the maximum 
indentation depth, as obtained from OVITO
and reported in our previous work \cite{Javier2021}. 
The sample was slid on the (011) plane, revealing that 
the maximum strain follows the $\langle 111 \rangle$ 
slip directions, due to the BCC crystal geometry of the
W samples.
This highlights the importance of accurate modeling for 
simulations involving open boundaries.
From our MD simulations, the formation of indentation 
plastic imprints is a process associated to the onset 
of plastic bursts during mechanical loading 
that is modeled in similar manner by tabGAP, ABOP, and the 
modified 
EAM potential, where our results are in good agreement 
with experimental electron microscopy images 
\cite{YU2020135,1998562,Wangexp}. Results for both (011) and 
(111) orientations can be found in 
the supplementary material \cite{SM}.
In addition, the dynamics of twin nucleation and twin 
annihilation during the loading process is a key aspect of 
the plastic deformation of the W material
that needs to be observed in experimental nanoindentation 
test.
Twin nucleation refers to the process by which a twinned 
region forms within the W lattice, while twin annihilation 
refers to the process by which twinned regions transform into 
dislocations or a dislocation network beneath the 
indenter tip, as reported experimentally 
by Wang et al. \cite{sciadv.aay2792}
in compression experiments.
These processes are generally influenced by the surface 
energy of the sample, which is a measure of the energy 
required to create or modify the surface of the material 
by external load.
In our simulations, we utilized the BDA method 
\cite{moller2016bda} to identify material defects as twin planes 
{112}, as described in Appendix \ref{sec:appendix}.
Although some W atoms were identified as twins in all the 
simulations, consistent with the literature \cite{GOEL2018196}, 
they can be likely misidentified
as screw dislocations. 
Only in the tabGAP simulations, several W atoms were 
observed in the near vicinity of the indenter tip, which 
exhibited twin defects upon structural analysis and visual 
examination.
(See Fig \ref{fig:pattern300}f). 



\begin{figure}[!t]
   \centering
  % \includegraphics[width=0.40\textwidth]{Figures/dislocationNucleation.png}
  \includegraphics[width=0.45\textwidth,height=0.50\textwidth]{Figures/Fig9.png}
   \caption{(Color on-line). Visualization of the von Mises strain mapping
   for the indented [001] W sample at the maximum depth, 
   at room temperature. The W matrix is slid on the (011) 
   plane for better visualization. 
   BCC \{112\} twin boundaries
   are identified in our simulations 
   as depicted in f) 
   by BDA method} and are marked by white circles
   for the tabGAP simulations.
   \label{fig:pattern77}
\end{figure}


There are several machine learning-based interatomic potentials for W 
reported in literature, such as GAP \cite{Szlachta} and Spectral Neighbor 
Analysis Potential (SNAP) \cite{Wood}. 
However, nanoindentation simulations require simulation cells with millions
of atoms and open boundaries. A single MD simulation using GAP and SNAP
potentials would require a wall time of 10-20 days with high computational
resources demands, as we tested for our simulation cells. 
In our work, we are focused on modeling nanoindentation with interatomic 
potentials that offer the possibility of a good description of the plastic
deformation of W matrices with modest computer resources and wall times 
on the scale of hours. Therefore, we used a Linux cluster with 120 
Intel(R) Xeon(R) CPU E5-2680 v2 processors at 2.80GHz, with wall time of 
82 minutes for the EAM potential, 63 minutes for the EAM/ZBL potential, 
780 minutes for the MEAM potential, 960 minutes for the ABOP potential, 
and 1658 minutes for the tabGAP potential that seems to model several 
defect nucleation and evolution mechanisms.

